Uniform Complexity for Text Generation

Large language models (LLMs) have shown promising results in a wide array of generative NLP tasks, such as summarization and machine translation. In the context of narrative generation, however, existing models still do not capture factors that contribute to producing consistent text. For instance, it is logical that a piece of text or a story should be uniformly readable throughout and that this form of complexity should be controllable. As such, if the complexity of an input text prompt is rated first-grade reading level in the Flesch Reading Ease test, then the generated text continuing the plot should also be within this range of complexity. With this in mind, we introduce Uniform Complexity for Text Generation (UCTG), a new benchmark test which raises the challenge of making generative models observe uniform linguistic properties with respect to prompts. We experiment with over 150+ linguistically and cognitively motivated features for evaluating text complexity in humans and generative models. From our results, we find that models such as GPT-2 struggle to preserve the complexity of input prompts used in its generations, even if finetuned with professionally written texts.

==> placeholder.tex <==
%%
%% - SEMANTIC SIMILARITY TABLE
%%
\begin{table}[!htbp]
\small
\centering
\begin{tabular}{lcc}
\toprule
Model & {\bf SentenceSim}     & {\bf BERTScore}  \\
\midrule
Human       & 0.3963 & 0.8153 \\
GPT2        & 0.4343 & 0.8229 \\
GPT2-DF     & 0.3591 & 0.8204 \\
GPT2-UF     & 0.3873 & 0.8179 \\
\bottomrule
\end{tabular}
\caption{Top correlated complexity features of GPT-2 and finetuned GPT-2 model with human continuations.}
\label{tab:semsimilarity}
\end{table}




\section{Trade-Offs with Finetuning for Uniform Complexity}


On using BERTScore is task-agnostic.
"By taking this approach, it can be observed firstly if individual segments of the story are semantically linked back to the prompt, but also if each segment is semantically linked to the previous segment.

BERTScore looks at predicting whether each sentence in the story logically follows on from the prompt."

%% Results from ANOVA and Tukey's HSD
%% Semantic Similarity = p value is 1.1102e-16 (p<0.05), Tukey's HSD show that human vs GPT2-UF is non significant while the other iterations are significantly different (p<0.05).
%% BERScore = p value is 1.1102e-16 (p<0.05), Tukey's HSD show that ALL iterations are significantly different (p<0.05).
